Large Data and (Not Even Very) Complex Ecological Models: When Worlds Collide

We consider the challenges that arise when fitting complex ecological models to 'large' data sets. In particular, we focus on random effect models which are commonly used to describe individual heterogeneity, often present in ecological populations under study. In general, these models lead to a likelihood that is expressible only as an analytically intractable integral. Common techniques for fitting such models to data include, for example, the use of numerical approximations for the integral, or a Bayesian data augmentation approach. However, as the size of the data set increases (i.e. the number of individuals increases), these computational tools may become computationally infeasible. We present an efficient Bayesian model-fitting approach, whereby we initially sample from the posterior distribution of a smaller subsample of the data, before correcting this sample to obtain estimates of the posterior distribution of the full dataset, using an importance sampling approach. We consider several practical issues, including the subsampling mechanism, computational efficiencies (including the ability to parallelise the algorithm) and combining subsampling estimates using multiple subsampled datasets. We demonstrate the approach in relation to individual heterogeneity capture-recapture models. We initially demonstrate the feasibility of the approach via simulated data before considering a challenging real dataset of approximately 30,000 guillemots, and obtain posterior estimates in substantially reduced computational time.

==> references.tex <==
@Manual{rjags,
    title = {rjags: Bayesian Graphical Models using MCMC},
    author = {Martyn Plummer},
    year = {2016},
    note = {R package version 4-6},
    url = {https://CRAN.R-project.org/package=rjags},
  }



@inproceedings{nguyen2014improving,
  title={Improving {SMC} sampler estimate by recycling all past simulated particles},
  author={Nguyen, Thi Le Thu and Septier, Fran{\c{c}}ois and Peters, Gareth W and Delignon, Yves},
  booktitle={Statistical Signal Processing (SSP), 2014 IEEE Workshop on},
  pages={117--120},
  year={2014},
  organization={IEEE}
}
@article{ionides2008truncated,
  title={Truncated importance sampling},
  author={Ionides, Edward L},
  journal={Journal of Computational and Graphical Statistics},
  volume={17},
  number={2},
  pages={295--311},
  year={2008},
  publisher={Taylor \& Francis}
}

@article{vehtari2015pareto,
  title={Pareto smoothed importance sampling},
  author={Vehtari, Aki and Simpson, Daniel and Gelman, Andrew and Yao, Yuling and Gabry, Jonah},
  journal={arXiv:1507.02646},
  year={2015}
}


@article{elvira2020importance,
  title={Importance Gaussian Quadrature},
  author={Elvira, V. and Martino, L. and Closas, P.},
  journal={IEEE Transactions on Signal Processing},
  volume={69},
  pages={474--488},
  year={2020},
  publisher={IEEE}
}

@book{owen2013montecarlo,
   author = {A. Owen},
   year = 2013,
   title = {Monte Carlo theory, methods and examples},
    publisher={http://statweb.stanford.edu/$\sim$owen/mc/},
}


@article{luengo2018efficient,
  title={Efficient linear fusion of partial estimators},
  author={Luengo, David and Martino, Luca and Elvira, V{\'\i}ctor and Bugallo, M{\'o}nica},
  journal={Digital Signal Processing},
  volume={78},
  pages={265--283},
  year={2018},
  publisher={Elsevier}
}

@article{Douc07,
	Author = {R. Douc and A. Guillin and J. M. Marin and C. P. Robert},
	Journal = {ESAIM: Probability and Statistics},
	Pages = {427--447},
	Title = {Minimum variance importance sampling via Population {M}onte {C}arlo},
	Volume = {11},
	Year = {2007}
	}

@article{martino2018recycling,
  title={The recycling {G}ibbs sampler for efficient learning},
  author={Martino, Luca and Elvira, Victor and Camps-Valls, Gustau},
  journal={Digital Signal Processing},
  volume={74},
  pages={1--13},
  year={2018},
  publisher={Elsevier}
}

  @book{robert2012bayesian,
  title={Bayesian Ideas and Data Analysis},
  author={Robert, Christian and Christensen, Ronald and Johnson, Wesley and Branscum, Adam and Hanson, Timothy},
  year={2012},
  publisher={Taylor \& Francis Group}
}
  
@Manual{R,
    title = {R: A Language and Environment for Statistical Computing},
    author = {{R Core Team}},
    organization = {R Foundation for Statistical Computing},
    address = {Vienna, Austria},
    year = {2021},
    url = {https://www.R-project.org/},
  }

@article{lunn2000,
  title={Win{BUGS}: a {{Bayesian}} modelling framework: concepts, structure, and extensibility},
  author={Lunn, D. J. and Thomas, Andrew and Best, Nicky and Spiegelhalter, David},
  journal={Statistics and Computing},
  volume={10},
  pages={325--337},
  year={2000}
  }
  
  @article{schaub2004,
  title={Estimating survival and temporary emigration in the multistate capture-recapture framework},
  author={Schaub, M. and Giménez, O. and Benedikt, R.S. and Pradel, R.},
  journal={Ecology},
  volume={85},
  pages={2107--2113},
  year={2004}
  }
  
   @article{reynolds2009,
  title={Integrated data analysis in the presence of emigration and mark loss},
  author={Reynolds, T.J. and R. King and J. Harwood and M. Frederiksen and M.P. Harris and S. Wanless},
  journal={Journal of Agricultural, Biological, and Environmental Statistics},
  volume={14},
  number={},
  pages={411--431},
  year={2009}
  }
  
  @article{lebreton1999,
  title={Competing events, mixtures of information and multistratum recapture models},
  author={Lebreton, J. D. and Almeras, T. and Pradel, R.},
  journal={Bird Study},
  volume={46},
  number={},
  pages={39--46},
  year={1999}
  }
  
  @article{lunn2000b,
  title={{W}in{BUGS}: A {B}ayesian modelling framework: Concepts, structure, and extensibility},
  author={Lunn, David J and Thomas, Andrew and Best, Nicky and Spiegelhalter, David},
  journal={Statistics and computing},
  volume={10},
  pages={325--337},
  year={2000}
  }
  
  @article{carpenter,
  title={Stan: {A} probabilistic programming language},
  author={Carpenter, B. and Gelman, A. and Hoffman, M. D. and Lee, D. and Goodrich, B. and Bentancourt, M. and Brubaker, M. and Guo, J. and Riddell, A.},
  journal={Journal of Statistical Software},
  volume={76},
  number={1},
  pages={},
  year={2017}
  }
  
  @article{nimble,
  title={Programming With Models: {W}riting Statistical Algorithms for General Model Structures With {NIMBLE}},
  author={P. {de Valpine} and D. Turek and C. Paciorek and C. Anderson-Bergman and D. Lang and R. Bodik},
  journal={Journal of Computational and Graphical Statistics },
  volume={26},
  pages={403--413},
  year={2017},
}

@article{dev04,
  title={Monte {C}arlo state-space likelihoods by weighted posterior kernel density estimation},
  author={P. {de Valpine}},
  journal={Journal of the American Statistical Association},
  volume={99},
  number={},
  pages={523--534},
  year={2004},
}

@article{dev02,
  title={Review of methods for fitting time-series models with process and observation error and likelihood calculations for nonlinear, non-{G}aussian state-space models},
  author={P. {de Valpine}},
  journal={Bulletin of Marine Science},
  volume={70},
  number={},
  pages={455--471},
  year={2002},
}

@article{coua99,
  title={The Use of Mixed Logit Models to Reflect Heterogeneity in Capture-Recapture Studies},
  author={Coull, B. A. and Agresti, A.},
  journal={Biometrics},
  volume={55},
  pages={294--301},
  year={1999},
}

  
  @inproceedings{plummer2003jags,
  title={{JAGS}: A program for analysis of {B}ayesian graphical models using {G}ibbs sampling},
  author={Plummer, M.},
  booktitle={Proceedings of the 3rd international workshop on distributed statistical computing},
  volume={124},
  pages={1--9},
  year={2003}
}
 
@article{Smout2011,
  title={Estimating survival and temporary emigration in the multistate capture-recapture framework},
  author={Smout, S. and King, R. and Pomeroy, P.},
  journal={Environmental and Ecological Statatistics},
  volume={18},
  number={},
  pages={331--347},
  year={2011}
  }
  
@article{kendall1997,
  title={Estimating temporary emigration using capture-recapture data with {P}ollock’s robust design},
  author={Kendall, W. L. and Nichols, J. D. and Hines, J.E.},
  journal={Ecology},
  volume={78},
  number={},
  pages={563--578},
  year={1997}
  }

@TechReport{brooks2004,
    address = {Kent, {UK}},
    type = {},
    title = {Recent progress in using marked individuals to understand animal population biology},
    url = {},
    author = {Brooks, S.P. and Catchpole, E.A. and Coulson, T. and Lebreton, J.D. and Morgan, B.J.T.},
    year = {2004},
    institution = {University of {K}ent, {C}anterbury},
  }

@TechReport{RMark,
    address = {Seattle, {WA}},
    type = {{AFSC} Processed Rep.},
    title = {{RMark}: An {R} {I}nterface for {A}nalysis of {C}apture-{R}ecapture {D}ata with {MARK}},
    url = {http://www.afsc.noaa.gov/Publications/ProcRpt/PR2013-01.pdf},
    number = {2013-01},
    author = {J. L. Laake},
    year = {2013},
    institution = {Alaska Fish. Sci. Cent., {NOAA}, Natl. Mar. Fish. Serv.},
  }
  
@book{gelman2014bayesian,
  title={Bayesian {D}ata {A}nalysis},
  author={Gelman, Andrew and Carlin, John B and Stern, Hal S and Rubin, Donald B},
  volume={2},
  year={2014},
  publisher={Chapman \& Hall/CRC Boca Raton, FL, USA}
}

@book{king2010bayesian,
  title={Bayesian {A}nalysis for {P}opulation {E}cology},
  author={King, Ruth and Morgan, B. J. T. and Giménez, Olivier and Brooks, S. P.},
  year={2010},
  publisher={CRC Press}
}

@book{kery2011bayesian,
  title={Bayesian Population Analysis using WinBUGS: A hierarchical perspective},
  author={K{\'e}ry, Marc and Schaub, Michael},
  year={2011},
  publisher={Academic Press}
}

@incollection{gimenez2009weak,
  title={Weak identifiability in models for mark-recapture-recovery data},
  author={Gimenez, Olivier and Morgan, B. J. T. and Brooks, S. P.},
  booktitle={Modeling demographic processes in marked populations},
  pages={1055--1067},
  year={2009},
  publisher={Springer}
}

@article{cole2010determining,
  title={Determining the parametric structure of models},
  author={Cole, Diana J and Morgan, Byron JT and Titterington, DM},
  journal={Mathematical biosciences},
  volume={228},
  number={1},
  pages={16--30},
  year={2010}}

@article{garrett2000latent,
  title={Latent class model diagnosis},
  author={Garrett, Elizabeth S and Zeger, Scott L},
  journal={Biometrics},
  volume={56},
  number={4},
  pages={1055--1067},
  year={2000}}

@book{newman2014,
  title={Modelling Population Dynamics: {M}odel Formulation, Fitting and Assessment using State-Space Methods},
  author={Newman, K. and Buckland, S. and Morgan, B. and King, R. and Borchers, D. and Cole, D. and Besbeas, P. and Giménez, O. and Thomas, L. },
  year={2014},
  publisher={Springer}
}

@article{halley1995,
  title={Colony attendance patterns and recruitment in inmature Common Murres (\textit{Uria aalge})},
  author={Halley, D. J. and Harris, M. P. and Wanless, S.},
  journal={The Auk},
  volume={112},
  number={4},
  pages={647--957},
  year={1995}}

@article{harris96a,
  title={Philopatry in the {C}ommon {M}urre},
  author={Harris, M. P. and Halley, D. J. and Wanless, S.},
  journal={Bird Study},
  volume={43},
  number={},
  pages={134--137},
  year={1996}
  }
  
  @book{seber19,
  title={Capture-Recapture: Parameter Estimation for Open Animal Populations},
  author={Seber, G.A.F. and Schofield, M.R.},
  year={2019},
  publisher={Springer}
	}


  


@article{burnham2002evaluation,
  title={Evaluation of some random effects methodology applicable to bird ringing data},
  author={Burnham, Kenneth P. and White, Gary C.},
  journal={Journal of applied statistics},
  volume={29},
  number={1-4},
  pages={245--264},
  year={2002}}
  
  @article{Mark,
author = {Gary C.  White  and  Kenneth P.   Burnham },
title = {Program {MARK}: survival estimation from populations of marked animals},
journal = {Bird Study},
volume = {46},
number = {sup1},
pages = {S120--S139},
year  = {1999},
publisher = {Taylor & Francis},
doi = {10.1080/00063659909477239},
URL = { https://doi.org/10.1080/00063659909477239
  },
eprint = { https://doi.org/10.1080/00063659909477239},
}


@article{mccrea2010,
  title={Multi-Site Integrated Population Modelling},
  author={McCrea, R. and Morgan, B. J. T. and Giménez, O. and Besbeas, P. B.},
  journal={Journal of Agricultural, Biological, and Environmental Statistics},
  volume={15},
  number={},
  pages={539--561},
  year={2010}}
  
  @article{mccrea2012,
  title={Model comparison and assessment for multi-state
capture-recapture-recovery models},
  author={McCrea, R. and Morgan, B. J. T. and Giménez, O. and Bregnballe, T.},
  journal={Journal of Ornithology},
  volume={152},
  number={Suppl.2},
  pages={293--303},
  year={2012}}
  
  @article{lack1946,
  title={Do juvenile birds survive less well than adults?},
  author={Lack, D.},
  journal={British Birds},
  volume={39},
  number={},
  pages={258--264},
  year={1946}}
  
  @inproceedings{Haldane55,
  author={Haldane, J. B. S},
  title={The calculation of mortality rate from ringing data},
  booktitle={Proceedings of the 11th International Orinthological Congress, Basel},
  volume ={11},
  pages={154--458},
  year={1955}
  }
  
 
@article{Seber1971,
  title={Estimating age-specific survival rates from bird-band returns when the reporting rate is constant},
  author={Seber, G.A.F.},
  journal={Biometrika},
  volume={58},
  number={},
  pages={491--497},
  year={1971}
  }

@article{Barker1997,
  title={Joint Modeling of Live-Recapture, Tag-Resight, and Tag-Recovery Data},
  author={Barker, R.J.},
  journal={Biometrics},
  volume={53},
  number={2},
  pages={666--677},
  year={1997}
  }

  @article{Barker1999,
  title={Joint analysis of mark-recapture, resighting and ring-recovery data with age-dependence and marking-effect},
  author={Barker, R.J.},
  journal={Bird Study},
  volume={46},
  number={},
  pages={82--91},
  year={1999}
  }

  
@article{lebreton1995,
  title={A Simultaneous Survival Rate Analysis of Dead Recovery and Live Recapture Data},
  author={Lebreton, J. D and Morgan, B. J. T. and Pradel, R. and Freeman, S. N.},
  journal={Biometrics},
  volume={51},
  number={4},
  pages={1418--1428},
  year={1995}
  }


@book{McCrea,
  title={Analysis of Capture-Recapture Data},
  author={McCrea, R. and Morgan, B. J. T.},
  year={2015},
  publisher={CRC Press}
	}

@article{natarajan1995note,
  title={A note on the existence of the posterior distribution for a class of mixed models for binomial responses},
  author={Natarajan, Ranjini and McCulloch, Charles E},
  journal={Biometrika},
  pages={639--643},
  year={1995}
}

@article{cole2012determining,
  title={Determining parameter redundancy of multi-state mark--recapture models for sea birds},
  author={Cole, Diana J},
  journal={Journal of Ornithology},
  volume={152},
  number={2},
  pages={305--315},
  year={2012}
}

@article{croxall1991population,
  title={Population regulation of seabirds: implications of their demography for conservation},
  author={Croxall, JP and Rothery, P},
  journal={Bird population studies: relevance to conservation and management. Oxford University Press, Oxford},
  pages={272--296},
  year={1991}
}

@article{votier2008recruitment,
  title={Recruitment and survival of immature seabirds in relation to oil spills and climate variability},
  author={Votier, Stephen C and Birkhead, Tim R and Oro, Daniel and Trinder, Mark and Grantham, MJ and Clark, Jacquie A and McCleery, Robin H and Hatchwell, Ben J},
  journal={Journal of Animal Ecology},
  volume={77},
  number={5},
  pages={974--983},
  year={2008}
}

@article{birkhead77,
  title={Population parameters for the Common Murre \textit{Uria aalge}},
  author={Birkhead, T. R. and P. J. Hudson},
  journal={Ornis Scandinavica},
  volume={},
  number={},
  pages={145--154},
  year={1977}
}

@article{brooks2000bayesian,
  title={Bayesian animal survival estimation},
  author={Brooks, S. P. and Catchpole, Edward A. and Morgan, B. J. T.},
  journal={Statistical Science},
  volume={56},
  number={},
  pages={357--376},
  year={2000}
}

@article{Catchpole97,
  title={Detecting parameter redundancy},
  author={E.A. Catchpole and B. J. T. Morgan},
  journal={Biometrika},
  volume={84},
  number={},
  pages={187--196},
  year={1997}
}

@article{Catchpole98,
  title={Integrated Recovery/Recapture Data Analysis},
  author={E.A. Catchpole and S. N. Freeman and B. J. T. Morgan and M. P. Harris},
  journal={Biometrics},
  volume={54},
  number={},
  pages={33--46},
  year={1998}
}

@article{Greenwood,
  title={The natal and breeding dispersal of birds},
  author={P. J. Greenwood and P. H. Harvey},
  journal={Annual Review of Ecology, Evolution, and Systematics},
  volume={13},
  number={},
  pages={1--21},
  year={1982}
}


@incollection{Burnham93,
 author = {Burnham, K.P.},
 title  = {A theory for Combined Analysis of Ring Recovery and Recapture Data},
 booktitle = {Marked Individuals in the Study of Bird Population},
 editor = {Lebreton, J.D. and North, P. M.},
 year = {1993},
 pages = {199--213},
 numpages = {14},
 publisher = {Birkhäuser Verlag Basel},
 address = {Switzerland},
}

@article{harris2000survival,
  title={Survival of adult Common Guillemots \textit{Uria aalge} at three {S}cottish colonies},
  author={Harris, MIKE P and Wanless, SARAH and Rothery, PETER and Swann, ROBERT L and Jardine, DAVID},
  journal={Bird Study},
  volume={47},
  number={},
  pages={1--7},
  year={2000}
}


@article{Sarzo19,
  title={Bayesian immature survival analysis of the largest colony of {C}ommon murre \textit{{U}ria aalge} in the {B}altic sea},
  author={Sarzo, B. and Armero, C. and Conesa, D. and Hentati-Sundberg, J. and Olsson, O.},
  journal={Waterbirds},
  volume={42},
  number={},
  pages={304--313},
  year={2019}
	}

@article{Sarzo21,
  title={Correcting bias in survival probabilities for partially monitored populations via integrated models},
  author={Sarzo, B. and King, R. and Conesa, D. and Hentati-Sundberg, J.},
  journal={Journal of Agricultural, Biological and Environmental Statistics},
  volume={26},
  number={2},
  pages={200--219},
  doi={10.1007/s13253-020-00423-1},
  year={2021}
	}


@article{hubbard14,
  title={Parameter redundancy in capture-recapture-recovery
models},
  author={Hubbard, B. A. and D. J. Cole and B. J. T. Morgan},
  journal={Statistical Methodology},
  volume={17},
  number={},
  pages={17--29},
  year={2014}
}

@article{osterblom04,
  title={Adult survival and avian cholera in {C}ommon {G}uillemots \textit{{U}ria aalge} in the {B}altic {S}ea},
  author={\"{O}sterblom, H. and Van der Jeugd, H. P. and Olsson, O.},
  journal={Ibis},
  volume={146},
  number={},
  pages={1--4},
  year={2004}
  }
  
  @incollection{Francis09,
  author      = {Francis, C. M. and Saurola, P.},
  title       = {Estimating Demographic Parameters from Complex Data Sets: {A} Comparison of Bayesian Hierarchical and Maximum-Likelihood Methods for Estimating Survival Probabilities of Tawny Owls, \textit{Strix aluco} in {F}inland},
  editor      = {Thomson, D. L. and Cooch, E. G. and Conroy, M. J.},
  booktitle   = {Modeling Demographic Processes In Marked Populations},
  publisher   = {Springer},
  address     = {Boston, MA},
  year        = {2009},
  pages       = {617--637}
}

@article{Hestbeck91,
author = {Hestbeck, Jay B. and Nichols, James D. and Malecki, Richard A.},
title = {Estimates of Movement and Site Fidelity Using Mark-Resight Data of Wintering Canada Geese},
journal = {Ecology},
volume = {72},
pages = {523-533},
doi = {10.2307/2937193},
year = {1991}
}
  
  @article{gimenez2007state,
  title={State-space modelling of data on marked individuals},
  author={Gimenez, O. and Rossi, V. and Choquet, R. and Dehais, C. and Doris, B. and Varella, H. and Vila, J. P. and Pradel, R.},
  journal={Ecological Modelling},
  volume={206},
  pages={431--438},
  year={2007}
}

@article{gimenez10,
  title={Individual heterogeneity in studies on marked animals using
numerical integration: capture-recapture mixed models},
  author={Gimenez, O. and Choquet, R. },
  journal={Ecology},
  volume={91},
  pages={951--957},
  year={2010}
}


@article{royle2008modeling,
  title={Modeling individual effects in the {C}ormack--{J}olly--{S}eber model: {A} state--space formulation},
  author={Royle, J Andrew},
  journal={Biometrics},
  volume={64},
  pages={364--370},
  year={2008}
}

@article{jolly1965,
  title={Explicit estimates from capture-recapture data with both death and immigration-stochastic model},
  author={Jolly, G.M.},
  journal={Biometrika},
  volume={52},
  number={},
  pages={225--247},
  year={1965}
	}
	
@article{seber1965,
  title={A note on the multiple recapture census},
  author={Seber, G.A.F.},
  journal={Biometrika},
  volume={52},
  number={},
  pages={249--259},
  year={1965}
	}
	
	@article{barker2004,
  title={Encounter history modelling of joint mark-recapture, tag-resighting and tag-recovery data under temporary emigration},
  author={Barker, R.J. and Burnham, K. P. and White, G.},
  journal={Statistica Sinica},
  volume={14},
  number={},
  pages={1037--1055},
  year={2004}
	}

@article{cormack1964,
  title={Estimates of survival from the sighting of marked animals},
  author={Cormack, R.M.},
  journal={Biometrika},
  volume={51},
  pages={429--438},
  year={1964}
	}
	 
@article{king2003,
  title={Closed-form likelihoods for {A}rnason-{S}chwarz models},
  author={King, Ruth and Brooks, S. P.},
  journal={Biometrika},
  volume={90},
  number={},
  pages={435--444},
  year={2003}
}

@article{king14,
  title={Statistical {E}cology},
  author={King, Ruth},
  journal={Annual Review of Statistics and its Application},
  volume={1},
  number={},
  pages={401--426},
  year={2014}
}

@article{king2014,
  title={A generalised likelihood framework for partially
observed capture-recapture-recovery models},
  author={King, Ruth and McCrea, R.},
  journal={Statistical Methodology},
  volume={17},
  number={},
  pages={30--45},
  year={2014}
}

@article{colchero2012,
  title={Bayesian inference on age-specific survival for censored and truncated data},
  author={Colchero, F. and Clark, J.S.},
  journal={Journal of Animal Ecology},
  volume={81},
  number={},
  pages={139--149},
  year={2012}
}

@article{bonner2010,
  title={Continuous Covariates in Mark-Recapture-Recovery Analysis: A Comparison of Methods},
  author={Bonner, S. and B. J. T. Morgan and King, R.},
  journal={Biometrics},
  volume={66},
  number={},
  pages={1256--1265},
  year={2010}
}

@article{bonner2013,
  title={Implementing the trinomial mark–recapture–recovery
model in PROGRAM {MARK}},
  author={Bonner, S. },
  journal={Methods in Ecology and Evolution},
  volume={4},
  number={},
  pages={95--98},
  year={2013}
}
@article{king2012review,
  title={A review of {B}ayesian state-space modelling of capture--recapture--recovery data},
  author={King, Ruth},
  journal={Interface Focus},
  volume={2},
  number={},
  pages={190--204},
  year={2012}
}

@article{robert2011short,
  title={A short history of {M}arkov Chain {M}onte {C}arlo: {S}ubjective recollections from incomplete data},
  author={Robert, Christian and Casella, George},
  journal={Statistical Science},
  volume={26},
  number={},
  pages={102--115},
  year={2011}
}

@article{harris2007within,
  title={Within-and between-year variation in the juvenile survival of Common Guillemots \textit{Uria aalge}},
  author={Harris, Michael P and Frederiksen, Morten and Wanless, Sarah},
  journal={Ibis},
  volume={149},
  number={},
  pages={472--481},
  year={2007}
}

@article{sandvik2008high,
  title={High survival of immatures in a long-lived seabird: insights from a long-term study of the Atlantic puffin (Fratercula arctica)},
  author={Sandvik, Hanno and Erikstad, Kjell Einar and Fauchald, Per and Tveraa, Torkild},
  journal={The Auk},
  volume={125},
  pages={723--730},
  year={2008}
}

@article{olsson2017,
  title={Population trends and status of four seabird species (\textit{Uria aalge}, \textit{Alca torda}, \textit{Larus fuscus}, \textit{Larus argentatus}) at {S}tora {K}arls\"{o} in the {B}altic Sea},
  author={Olsson, O. and J. Hentati-Sundberg},
  journal={Ornys Svecica},
  volume={27},
  number={},
  pages={64--93},
  year={2017}
}


@article{crespin2006recruitment,
  title={Recruitment to a seabird population depends on environmental factors and on population size},
  author={Crespin, Laurent and Harris, Michael P and Lebreton, Jean-Dominique and Frederiksen, Morten and Wanless, Sarah},
  journal={Journal of Animal Ecology},
  volume={75},
  pages={228--238},
  year={2006}
}


@misc{thomas2004openbugs,
  title={OpenBUGS},
  author={Thomas, Andrew and O’Hara, Robert B},
  year={2004}
}

@inproceedings{plummer2003jagsB,
  	title={{JAGS}: {A} program for analysis of {B}ayesian graphical models using {G}ibbs sampling},
  	author={Plummer, Martyn},
 	 booktitle={Proceedings of the 3rd international workshop on distributed statistical computing},
 	 volume={124},
  	pages={1--9},
  	year={2003}
	}
  
  @book{lesaffre2012bayesian,
  title={Bayesian biostatistics},
  author={Lesaffre, Emmanuel and Lawson, Andrew B},
  year={2012},
  publisher={John Wiley \& Sons}
}

@book{roylebook,
  title={Hierarchical modelling and inference in {E}cology},
  author={Royle, J. A. and Dorazio, R. M.},
  year={2008},
  publisher={Elsevier}
}

@book{Nettleship85,
  title={The {A}tlantic {A}lcidae: the {E}volution, {D}istribution and {B}iology of the {A}uks {I}nhabiting the {A}tlantic {O}cean and
{A}djacent {W}ater {A}reas},
  author={Nettleship, D. N. and T. R. Birkhead},
  year={1995},
  publisher={Academic Press}
}

@article{lebreton1992modeling,
      title={Modeling survival and testing biological hypotheses using marked animals: {A} unified approach with case studies},
      author={Lebreton, Jean Dominique and Burnham, Kenneth P and Clobert, Jean and Anderson, David R},
      journal={Ecological Monographs},
      volume={62},
      number={},
      pages={67--118},
      year={1992},
      publisher={Wiley Online Library}
}

@article{langrock13,
      title={Maximum likelihood estimation of Mark-Recapture-Recovery models in the presence of continuous covariates},
      author={Langrock, R. and King, R.},
      journal={Annals of Applied Statistics},
      volume={7},
      number={},
      pages={1709--1732},
      year={2013},
}

@article{Worthington14,
      title={Analysing Mark-recapture-recovery Data in the Presence of Missing Covariate data via Multiple Imputation},
      author={Worthington, H. and King, R. and Buckland, S. T.},
      journal={Journal of Agricultural, Biological, and Environmental Statistics},
      volume={20},
      number={},
      pages={28--46},
      year={2015},
}

@article{kendall2002,
      title={Estimating state-transition probabilities for unobservable states using capture-recapture/resighting data},
      author={Kendall, W. L. and Nichols, J. D.},
      journal={Ecology},
      volume={83},
      pages={3276--3284},
      year={2002},
}
@article{cathpole2008,
      title={A new method for analysing discrete life history data with missing covariate values},
      author={Catchpole, E. A. and Morgan, B. J. T. and Tavecchia, J.},
      journal={Journal of the Royal Statistical Society: Series B},
      volume={70},
      number={},
      pages={445--460},
      year={2008},
}

@article{stahl2006relative,
  title={Relative importance of avian life-history variables to population growth rate},
  author={Stahl, Justyn T and Oli, Madan K},
  journal={Ecological Modelling},
  volume={198},
  pages={23--39},
  year={2006},
  publisher={Elsevier}
}

@article{sanz2016estimating,
  title={Estimating recruitment and survival in partially monitored populations},
  author={Sanz-Aguilar, Ana and Igual, Jos{\'e} Manuel and Oro, Daniel and Genovart, Meritxell and Tavecchia, Giacomo},
  journal={Journal of Applied Ecology},
  volume={53},
  pages={73--82},
  year={2016},
  publisher={Wiley Online Library}
}

@mastersthesis{kadin2007post,
  title={Post-fledging survival and sexual maturation in Common guillemots \textit{{U}ria aalge}--the influence of biological and ecological factors},
  author={Kadin, M.},
  school={Department of Systems Ecology, Stockholm University},
  address={Stockholm},
  year={2007}
}

@article{oro2000determinants,
  title={Determinants of local recruitment in a growing colony of {A}udouin's gull},
  author={Oro, Daniel and Pradel, Roger},
  journal={Journal of Animal Ecology},
  volume={69},
  number={},
  pages={119--132},
  year={2000},
  publisher={Wiley Online Library}
}

@article{dittmann2005dispersal,
  title={Dispersal decisions: common terns, Sterna hirundo, choose between colonies during prospecting},
  author={Dittmann, Tobias and Zinsmeister, Daniela and Becker, Peter H},
  journal={Animal Behaviour},
  volume={70},
  pages={13--20},
  year={2005},
  publisher={Elsevier}
}

@article{pradel2005,
  title={Multievent: An Extension of Multistate Capture-Recapture Models to Uncertain States},
  author={Pradel, R.},
  journal={Biometrics},
  volume={61},
  number={},
  pages={442--447},
  year={2005},
}


@inproceedings{golchi2016informative,
  title={Informative Priors and Bayesian Computation},
  author={Golchi, Shirin},
  booktitle={Data Science and Advanced Analytics (DSAA), 2016 IEEE International Conference on},
  pages={782--789},
  year={2016},
  organization={IEEE}
}

@book{christensen2011bayesian,
  title={Bayesian ideas and data analysis: an introduction for scientists and statisticians},
  author={Christensen, Ronald and Johnson, Wesley and Branscum, Adam and Hanson, Timothy E},
  year={2011},
  publisher={CRC Press}
}

@article{king2008,
  title={Analysing Complex Capture-Recapture Data: Incorporating Time-varying Covariate Information},
  author={King, R. and Brooks, S. P. and Coulson, T.},
  journal={Biometrics},
  volume={64},
  number={},
  pages={1187--1195},
  year={2008},
}

@book{hanmn19,
  title={Sampling Theory},
  author={Hankin, D. and Mohr, M. and Newman, K.},
  year={2019},
  publisher={Oxford University Press}
}

@article{besfmc02,
  title={Integrating mark-recapture-recovery
and census data to estimate animal abundance and demographic parameters},
  author={Besbeas, P. and Freeman, S. N. and Morgan, B. J. T. and Catchpole, E. A.},
  journal={Biometrics},
  volume={58},
  number={},
  pages={540--547},
  year={2002},
}

@article{herkk21,
title = {Laplace Approximations for Individual Heterogeneity Capture-Recapture Models},
author = {Herliansyah, R. and King, R. and King, S. E.},
year = {2022},
journal={Journal of Agricultural, Biological, and Environmental Statistics},
note = {in press}
}


@article{kinb08,
	title = {On the {Bayesian} {estimation} of a {closed} {population} {size} in the {presence} of {heterogeneity} and {model} {uncertainty}},
	volume = {64},
	journal = {Biometrics},
	author = {King, R. and Brooks, S. P.},
	year = {2008},
	pages = {816--824}
}

@article{ple00,
	title = {Unified maximum likelihood estimates for closed capture-recapture models using mixtures},
	volume = {56},
	journal = {Biometrics},
	author = {Pledger, S.},
	year = {2000},
	pages = {434--442}
}
 

@article{plepn03,
	title = {Open capture-recapture models with heterogeneity. {I} {C}ormack-{J}olly-{S}eber},
	volume = {59},
	journal = {Biometrics},
	author = {Pledger, S. and Pollock, K. H. and Norris, J. L.},
	year = {2003},
	pages = {786--794}
}

@article{kinmkb16,
	title = {Capture-recapture abundance estimation using a semi-complete data likelihood approach},
	volume = {10},
	journal = {The Annals of Applied Statistics},
	author = {King, Ruth and McClintock, Brett T. and Kidney, Darren and Borchers, David},
	year = {2016},
	pages = {264--285}
}

@article{gimcg17,
    title = {Individual heterogeneity and capture–recapture models: what, why and how?},
    author = {Gimenez, O. and Cam, E. and Gaillard J-M.},
    year = {2017},
    journal = {Oikos},
    volume = {127},
    pages = {664--686}
}


 @incollection{gimenez09,
  author      = {Gimenez, O. and Bonner, S. and King, R. and Parker, R. A. and Brooks, S. P. and Jamieson, L. E. and Grosbois, V. and Morgan, B. J. T. and Thomas, L.},
  title       = {Win{BUGS} for Population Ecologists: {B}ayesian Modelling using {M}arkov chain {M}onte {C}arlo ({MCMC}) Methods},
  editor      = {Thomson, D. L. and Cooch, E. G. and Conroy, M. J.},
  booktitle   = {Modeling Demographic Processes In Marked Populations},
  publisher   = {Springer},
  address     = {Boston, MA},
  year        = {2009},
  pages       = {885--918}
}


 @incollection{whibb09,
  author      = {White, G. C. and Burnham, K. P. and Barker, R. J.},
  title       = {Evaluation of a {B}ayesian {MCMC} Random Effects Inference Methodology for Capture-Mark-Recapture Data},
  editor      = {Thomson, D. L. and Cooch, E. G. and Conroy, M. J.},
  booktitle   = {Modeling Demographic Processes In Marked Populations},
  publisher   = {Springer},
  address     = {Boston, MA},
  year        = {2009},
  pages       = {1119--1127}
}

@book{mcmc,
editor = {Brooks, S. P. and Gelman, A. and Jones, G. and Meng, X.},
title = {Handbook of Markov Chain Monte Carlo; Methods and Applications},
year = {2011},
publisher = {CRC Press}
}

@article{tokk10,
author = {Tokdar,S. T. and Kass, R. E.},
title = {Importance sampling: a review},
year = {2010},
journal = {Wiley Interdisciplinary Reviews: Computational Statistics},
volume = {2},
pages = {54--60}
}

@article{robert2018accelerating,
author = {Robert, C. P. and Elvira, V. and Tawn, N. and Wu, C.},
title = {Accelerating {MCMC} algorithms},
year = {2018},
journal = {Wiley Interdisciplinary Reviews: Computational Statistics},
volume = {10},
pages = {1--14}
}

@article{elvm21,
author = {Elvira, V. and Martino, L. },
title = {Advances in Importance Sampling},
year = {2021},
journal = {Wiley StatsRef: Statistics Reference Online},
pages = {1--14}
}

@article{van21,
  title={{B}ayesian statistics and modelling},
  author={van de Schoot, Rens and Depaoli, Sarah and King, Ruth and Kramer, Bianca and M{\"a}rtens, Kaspar and Tadesse, Mahlet G and Vannucci, Marina and Gelman, Andrew and Veen, Duco and Willemsen, Joukje and Yau, Christopher},
  journal={Nature Reviews Methods Primers},
  volume={1},
  pages={1--26},
  year={2021},
  publisher={Nature Publishing Group}
}

@article{tran16,
      title={Importance sampling squared for {B}ayesian inference in latent variable models}, 
      author={Minh-Ngoc Tran, and Marcel Scharth, and Michael K. Pitt, and Robert Kohn},
      year={2016},
      eprint={1309.3339},
      journal={arXiv:1309.3339},
      primaryClass={stat.ME}
}


@article{Andrieu_2010,
	title = {Particle {Markov} chain {Monte} {Carlo} methods},
	volume = {72},
	issn = {13697412, 14679868},
	language = {English},
	urldate = {2020-03-20},
	journal = {Journal of the Royal Statistical Society: Series B},
	author = {Andrieu, Christophe and Doucet, Arnaud and Holenstein, Roman},
	year = {2010},
	pages = {269--342}
}

@article{Andrieu_2009,
	title = {The Pseudo-Marginal Approach for Efficient {Monte} {Carlo} {Computations}},
	volume = {37},
	issn = {0090-5364},
	urldate = {2020-03-23},
	journal = {The Annals of Statistics},
	author = {Andrieu, Christophe and Roberts, Gareth O.},
	year = {2009},
	pages = {697--725},
}
@book{mcbook,
   author = {Art B. Owen},
   year = 2013,
   title = {Monte Carlo theory, methods and examples}
}

@article{bar17, 
author = {Bardenet, R\'{e}mi and Doucet, Arnaud and Holmes, Chris}, 
title = {On {M}arkov Chain {M}onte {C}arlo Methods for Tall Data}, 
year = {2017}, 
volume = {18}, number = {1}, issn = {1532-4435}, abstract = {Markov chain Monte Carlo methods are often deemed too computationally intensive to be of any practical use for big data applications, and in particular for inference on datasets containing a large number n of individual data points, also known as tall datasets. In scenarios where data are assumed independent, various approaches to scale up the Metropolis-Hastings algorithm in a Bayesian inference context have been recently proposed in machine learning and computational statistics. These approaches can be grouped into two categories: divide-and-conquer approaches and, subsampling-based algorithms. The aims of this article are as follows. First, we present a comprehensive review of the existing literature, commenting on the underlying assumptions and theoretical guarantees of each method. Second, by leveraging our understanding of these limitations, we propose an original subsampling-based approach relying on a control variate method which samples under regularity conditions from a distribution provably close to the posterior distribution of interest, yet can require less than O(n) data point likelihood evaluations at each iteration for certain statistical models in favourable scenarios. Finally, we emphasize that we have only been able so far to propose subsampling-based methods which display good performance in scenarios where the Bernstein-von Mises approximation of the target posterior distribution is excellent. It remains an open challenge to develop such methods in scenarios where the Bernstein-von Mises approximation is poor.}, 
journal = {Journal of Machine Learning Research}, 
pages = {1515–1557}, 
numpages = {43} 
}
